Investigating Generalisation in Continuous Deep Reinforcement Learning

Deep Reinforcement Learning has shown great success in a variety of control tasks. However, it is unclear how close we are to the vision of putting Deep RL into practice to solve real world problems. In particular, common practice in the field is to train policies on largely deterministic simulators and to evaluate algorithms through training performance alone, without a train/test distinction to ensure models generalise and are not overfitted. Moreover, it is not standard practice to check for generalisation under domain shift, although robustness to such system change between training and testing would be necessary for real-world Deep RL control, for example, in robotics. In this paper we study these issues by first characterising the sources of uncertainty that provide generalisation challenges in Deep RL. We then provide a new benchmark and thorough empirical evaluation of generalisation challenges for state of the art Deep RL methods. In particular, we show that, if generalisation is the goal, then common practice of evaluating algorithms based on their training performance leads to the wrong conclusions about algorithm choice. Finally, we evaluate several techniques for improving generalisation and draw conclusions about the most robust techniques to date.

==> ICML19' (1)/ch4/corrcoef/corrcoef.tex <==
%\documentclass{article} 
%
%\begin{document}
%
%%\begin{tabular}{ l l l l l }
%%& obs& act& env & mdl\\
%%walker & -0.325& -0.382& & -0.172 &   \\
%%\end{tabular}
%
\begin{small}
\begin{sc}
\begin{tabular}{ l r r r r}
\toprule
& Obs. & Act.& Env. & Dom.\\
\midrule
Walker & -0.760& -0.722& -0.457 & -0.424 \\
Hopper & -0.203& -0.346& -0.473 & -0.415\\
HalfCheetah & -0.946& -0.843& -0.046 & -0.477\\
Pendulum & -0.132& -0.584& -0.665 & -0.630\\
D-Pendulum & -0.033& -0.732& ~0.025& ~0.324\\
\bottomrule\\
\end{tabular}
\end{sc}
\end{small}

%\end{document}

==> ICML19' (1)/ch4/table3a.tex <==
 \begin{table}[tb]
 \centering
 \caption{Improving Walker2d-PPO generalization  by training with noise. (a) Compares training return in deterministic ($\sigma_{tr} = 0.0$) and noisy  ($\sigma_{tr} = 0.2$) conditions. (b) Compares the testing performance of different training conditions. 
 \cut{Cols: Deterministic ($\sigma_{tr}=0.0$) vs noisy ($\sigma_{tr}=0.2$) training. Rows: Noise Types. Subrows: $\eta_{\sigma_{tr}}(\pi)$: Training return at noise level $\sigma_{tr}$. $\eta_{\sigma_{te}}(\pi)$: Testing return at noise $\sigma_{te}$.}`MDL' and `DOM' refer to training or testing on multiple domains respectively. For simplicity we overload $\sigma$ to refer to $\Sigma$ in the multi-domain  setting, and use $\eta_\sigma(\pi)$ to indicate expected return $\eta_{p(\Theta;\Sigma)}(\pi)$.}\label{table: noise}
\vspace{-0.2in}
\hspace{-0.15in} 
\begin{center}

\begin{small}
\begin{sc}
\subtable[Training performance $\eta_{\sigma_{tr}}$ of deterministic vs. noisy training]{
\resizebox{1.0\columnwidth}{!}{
\begin{tabular*}{\linewidth}{c c c}
\toprule
Train with $\sigma_{tr} = 0.0$& \multicolumn{2}{c}{Train with $\sigma_{tr} = 0.2$} \\ 
\midrule
Return $\eta_{\sigma_{tr}}(\pi) $  & Noise Type & Return $\eta_{\sigma_{tr}}(\pi) $\\
\midrule
\multirow{4}{*}{$3128.6 \pm 402.3$}  & Obs. & $1424.0 \pm 472.9$ \\
&Act. & $2694.8\pm504.9$\\
&Env. & $ 3261.3 \pm 436.5$ \\
& MDL. & $2445.3 \pm 631.0$ \\
\bottomrule
\end{tabular*}} \label{table: noise1}}
 \end{sc}
 \end{small}

\vspace{-0.2in}
\hspace{-0.1in} 
\begin{small}
\begin{sc}
\subtable[Testing performance $\eta_{\sigma_{te}}$ of deterministic vs. noisy training]{
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{l c c c c c }
\toprule
\multicolumn{2}{l}{\multirow{2}{*}{Noise Type}} & \multirow{2}{*}{$\sigma_{te}$}  & Train with  \cut{($\sigma_{tr} = 0.0$)} & Train with\\
& & & $\sigma_{tr} = 0.0$ & $\sigma_{tr} = 0.2$ \\
% && $\sigma_{te}$  & $\eta_{\sigma}(\pi)$ & $\eta_{\sigma}(\pi)$ \\
%& Training Return & $ \sigma_{te}$ &$\eta_{\sigma_{te}}(\pi)$ & Training Return & $ \sigma_{te}$ & $\eta_{\sigma_{te}}(\pi)$ \\
%\multirow{2}{*}{Noise Type}& \multicolumn{3}{c}{Training with Default Env ($\sigma_{tr} = 0.0s$)} &\multicolumn{3}{c}{Training in Noisy Environments ($\sigma_{tr} = 0.2$)}\\
%& Training Return & $ \sigma_{te}$ &$\eta_{\sigma_{te}}(\pi)$ & Training Return & $ \sigma_{te}$ & $\eta_{\sigma_{te}}(\pi)$ \\
\midrule
\multirow{3}{*}{Obs.}& \cut{\multirow{3}{*}{$\eta_{\sigma_{te}}(\pi)$}} & 0.0 & 3723.9$\pm$ 321.3  & 3682.9$\pm$415.6 \\
&& 0.2 & \textcolor{green}{2522.2 $\pm$593.4}  & \textcolor{green}{3036.1$\pm$576.3}\\
&& 0.4 & 937.8 $\pm$ 308.9 & 1303.8$\pm$374.5\\
\midrule
\multirow{3}{*}{Act.} &\cut{\multirow{3}{*}{$\eta_{\sigma_{te}}(\pi)$}}& 0.0 & 3678.8$\pm$355.5 &3596.5 $\pm$406.3\\
&& 0.2 & \textcolor{green}{2096.3$\pm$570.4} & \textcolor{green}{3044.0$\pm$525.6}\\
&& 0.4 & 919.7$\pm$249.5 & 1951.5$\pm$486.9\\
\midrule
\multirow{3}{*}{Env.} &\cut{\multirow{3}{*}{$\eta_{\sigma_{te}}(\pi)$}}& 0.0   &  3756.3$\pm$341.7 & 3761.8$\pm$415.1\\
&& 0.2 &  \textcolor{red}{3133.5$\pm$465.9} & \textcolor{red}{3225.4$\pm$450.0}\\
&& 0.4 & 2528.6$\pm$415.9	 & 2660.1 $\pm$ 436.1 \\
\midrule
\multirow{3}{*}{Dom.} &\cut{\multirow{3}{*}{$\eta_{\sigma_{te}}(\pi)$}}& 0.0   & 3725.1$\pm$343.7 & 3417.9$\pm$549.2\\
&& 0.2 & \textcolor{red}{3228.7$\pm$408.6} & \textcolor{red}{2985.2$\pm$486.4}\\
&& 0.4 & 2462.3$\pm$394.4 & 2468.2$\pm$341.9\\
\bottomrule
\end{tabular}} \label{table: noise2}}
\end{sc}
\end{small}
\end{center}
\vspace{-0.2in}
 \end{table}


==> ICML19' (1)/ch4/table4a.tex <==
% !TEX root = ../draft.tex
\begin{table*}[t!]
\tiny
\centering
\caption{Generalisation performance of basic Deep RL learners in terms of AUC scores. All settings are evaluated with 5 environments and 4 noise types in each environment. All results are averaged over 12 random seeds. Blue: Winning algorithm among the basic PPO, TRPO and DDPG baselines. Welch's t-test ($p<0.05$) is used for significance testing.}
\label{table: network1}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}


\begin{tabular}{l l c c c HHZ}
\toprule
\multicolumn{2}{l}{env. Name} & PPO & TRPO & DDPG & PPO-MDL & PPO-ObsNoise  \\
\midrule
Walker2d & obs. & \hblue{$\phantom{0}966.2 \pm 308.2$} & $\phantom{0}895.4 \pm 229.3$ & $\phantom{0}544.3 \pm 204.4$ & $\hgreen{1114.3\pm378.2}$ & $\hgreen{1455.8\pm388.9}$\\
& act. & $\phantom{0}845.5 \pm 251.4 $& \hblue{$1295.5 \pm 310.2$} &  $1115.2 \pm 531.1 $ &  \hgreen{$1082.1\pm349.6$} & $\hgreen{\mathbf{2078.3\pm522.8}}$\\
& env. & $2141.1 \pm 558.5$ & \hblue{$2653.6 \pm 402.3$} & $1550.5\pm 671.4$  & $2232.5\pm609.4$& $2301.8\pm521.0$\\
& dom. & $2114.3\pm567.2 $& \hblue{$2648.4 \pm 417.5$} & $1929.4\pm 839.8$ & $2232.9\pm601.8$ & $2313.7\pm521.9$ \\
\midrule
Hopper & obs. & $\phantom{0}592.6\pm 244.4$  & \hblue{$\phantom{0}643.8\pm 107.2$} &  $\phantom{0}352.7\pm245.5$  & $\hgreen{\phantom{0}733.5\pm143.4}$  & $\phantom{0}582.2\pm318.9$ \\
& act. & $\phantom{0} 609.0\pm167.6$ & \hblue{$\phantom{0}683.0\pm121.8$} & $\phantom{0}582.3\pm 163.9$ & $\hgreen{\phantom{0}905.8\pm143.4}$ & $\phantom{0}683.8\pm351.7$ \\
& env. & $1241.6\pm 438.7$ & \hblue{$1638.7\pm383.7$} &  $1042.2\pm337.9$& $\hgreen{1935.8\pm428.4}$ & $1164.9\pm804.3$\\
& dom. & \hblue{$1640.0\pm507.4$} & \hblue{$1622.6\pm 374.2$} & $1073.5\pm 358.3$ &  $\hgreen{1939.8\pm425.0}$ & $1167.8\pm813.6$ \\
\midrule
HalfCheetah & obs. & $1030.4\pm 133.9$ & $1045.9\pm \phantom{0} 444.6$ &  \hblue{$1152.7\pm361.0$} & $\hgreen{\mathbf{1629.6\pm\phantom{0}585.5}}$ & $\hgreen{\mathbf{1787.3\pm\phantom{0}562.8}}$ \\
& act. & $\phantom{0}773.1\pm177.5$ & $\phantom{0}906.1\pm   \phantom{0} 530.3$ & \hblue{$\phantom{0}943.6\pm312.8$}  & $\hgreen{1307.9\pm\phantom{0}498.9}$ & $\hgreen{\mathbf{1882.6\pm\phantom{0}627.2}}$\\
& env. & $1989.0\pm 658.2 $ & \hblue{$2322.0 \pm 1235.3$} & $1856.4 \pm 481.0$ & $1935.8\pm \phantom{0} 428.4$ & $1164.9\pm \phantom{0} 804.3$  \\
& dom. & $1871.0\pm583.5$ & \hblue{$2264.7\pm1191.2$} & $1963.9\pm451.7$ & $\hgreen{\mathbf{3748.2\pm1550.7}}$ & $\hgreen{\mathbf{3588.5\pm1020.7}}$\\
\midrule
Pendulum & obs. & $129.5\pm\phantom{0}32.5$ & \hblue{$182.8\pm 139.9$} & $\phantom{0}94.9\pm\phantom{0}33.1$  & $\hgreen{162.3\pm39.9}$ & $\phantom{0}54.1\pm\phantom{0}25.0$ \\
& act. & \hblue{$362.7\pm\phantom{0}43.7$} & $201.0\pm112.8$&$245.3\pm\phantom{0}85.3$ & $\hgreen{393.0\pm16.2}$ & $250.8\pm109.4$\\
& env. & \hblue{$995.4\pm\phantom{0}\phantom{0}8.0$} & $678.9\pm371.3$ & $607.2\pm280.0$  & $\hgreen{\mathbf{999.1\pm\phantom{0}2.4}}$ & $774.5\pm382.4$\\
& dom. & \hblue{$942.2\pm177.6$} & $676.1\pm370.9 $& $609.2\pm281.3$ &$\hgreen{\mathbf{999.3\pm\phantom{0}1.8}}$ & $775.0\pm381.8$ \\
\midrule
D-Pendulum & obs. & \hblue{$\phantom{0}923.3\pm\phantom{0}\phantom{0}61.5$} & $\phantom{0}715.1\pm\phantom{0}215.0$& $\phantom{0}525.4\pm257.9$  &$\hgreen{\mathbf{1071.8\pm\phantom{0}87.1}}$ & $\phantom{0}160.8\pm\phantom{0}13.9$ \\
& act. & \hblue{$2110.7\pm\phantom{0}\phantom{0}74.6$}& $1280.9\pm\phantom{0}286.4$ & $\phantom{0}962.4\pm178.7$  & $\hgreen{\mathbf{2161.5\pm\phantom{0}36.0}}$ & $\phantom{0}301.2\pm\phantom{0}64.6$ \\
& env. & \hblue{$7494.9\pm1189.1$} & $3023.9\pm\phantom{0}753.5$ & $2377.2\pm831.9$ & $\hgreen{\mathbf{8183.7\pm144.5}}$ & $\phantom{0}312.8\pm\phantom{0}50.5$ \\
& dom. & \hblue{$7013.8 \pm\phantom{0} 850.6$} & $6103.9\pm1530.1$ & $2215.8\pm 915.6$  &$\hgreen{\mathbf{8174.2\pm178.2}}$&$1178.9\pm688.1$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

==> ICML19' (1)/ch4/table4b.tex <==
% !TEX root = ../draft.tex


\begin{table*}[t!]
\tiny
\centering
\caption{Generalisation performance of training with noisy environments in terms of AUC score. All settings are evaluated with 5 environments and 4 noise types in each environment. All performance are averaged over 12 random seeds. Green: Noisy training settings that improve on corresponding PPO baseline. Welch's t-test ($p<0.05$) is used for significant testing.}
\label{table: network2}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}


\begin{tabular}{l l c H H c c}
\toprule
\multicolumn{2}{l}{env. Name} & PPO & TRPO & DDPG & PPO-MDL & PPO-ObsNoise  \\
\midrule
Walker2d & obs. & $\phantom{0}966.2 \pm 308.2$ & $\phantom{0}895.4 \pm 229.3$ & $\phantom{0}544.3 \pm 204.4$ & $\hgreen{1114.3\pm378.2}$ & $\hgreen{1455.8\pm388.9}$\\
& act. & $\phantom{0}845.5 \pm 251.4 $& \hblue{$1295.5 \pm 310.2$} &  $1115.2 \pm 531.1 $ &  \hgreen{$1082.1\pm349.6$} & $\hgreen{ {2078.3\pm522.8}}$\\
& env. & $2141.1 \pm 558.5$ & \hblue{$2653.6 \pm 402.3$} & $1550.5\pm 671.4$  & $2232.5\pm609.4$& $2301.8\pm521.0$\\
& dom. & $2114.3\pm567.2 $& \hblue{$2648.4 \pm 417.5$} & $1929.4\pm 839.8$ & $2232.9\pm601.8$ & $2313.7\pm521.9$ \\
\midrule
Hopper & obs. & $\phantom{0}592.6\pm 244.4$  & \hblue{$\phantom{0}643.8\pm 107.2$} &  $\phantom{0}352.7\pm245.5$  & $\hgreen{\phantom{0}733.5\pm143.4}$  & $\phantom{0}582.2\pm318.9$ \\
& act. & $\phantom{0} 609.0\pm167.6$ & \hblue{$\phantom{0}683.0\pm121.8$} & $\phantom{0}582.3\pm 163.9$ & $\hgreen{\phantom{0}905.8\pm143.4}$ & $\phantom{0}683.8\pm351.7$ \\
& env. & $1241.6\pm 438.7$ & \hblue{$1638.7\pm383.7$} &  $1042.2\pm337.9$& $\hgreen{1935.8\pm428.4}$ & $1164.9\pm804.3$\\
& dom. & $1640.0\pm507.4$ & \hblue{$1622.6\pm 374.2$} & $1073.5\pm 358.3$ &  $\hgreen{1939.8\pm425.0}$ & $1167.8\pm813.6$ \\
\midrule
HalfCheetah & obs. & $1030.4\pm 133.9$ & $1045.9\pm \phantom{0} 444.6$ &  \hblue{$1152.7\pm361.0$} & $\hgreen{ {1629.6\pm\phantom{0}585.5}}$ & $\hgreen{ {1787.3\pm\phantom{0}562.8}}$ \\
& act. & $\phantom{0}773.1\pm177.5$ & $\phantom{0}906.1\pm   \phantom{0} 530.3$ & \hblue{$\phantom{0}943.6\pm312.8$}  & $\hgreen{1307.9\pm\phantom{0}498.9}$ & $\hgreen{ {1882.6\pm\phantom{0}627.2}}$\\
& env. & $1989.0\pm 658.2 $ & \hblue{$2322.0 \pm 1235.3$} & $1856.4 \pm 481.0$ & $1935.8\pm \phantom{0} 428.4$ & $1164.9\pm \phantom{0} 804.3$  \\
& dom. & $1871.0\pm583.5$ & \hblue{$2264.7\pm1191.2$} & $1963.9\pm451.7$ & $\hgreen{ {3748.2\pm1550.7}}$ & $\hgreen{ {3588.5\pm1020.7}}$\\
\midrule
Pendulum & obs. & $129.5\pm\phantom{0}32.5$ & \hblue{$ {182.8\pm 139.9}$} & $\phantom{0}94.9\pm\phantom{0}33.1$  & $\hgreen{162.3\pm39.9}$ & $\phantom{0}54.1\pm\phantom{0}25.0$ \\
& act. & $362.7\pm\phantom{0}43.7$ & $201.0\pm112.8$&$245.3\pm\phantom{0}85.3$ & $\hgreen{ {393.0\pm16.2}}$ & $250.8\pm109.4$\\
& env. & $995.4\pm\phantom{0}\phantom{0}8.0$ & $678.9\pm371.3$ & $607.2\pm280.0$  & $\hgreen{ {999.1\pm\phantom{0}2.4}}$ & $774.5\pm382.4$\\
& dom. & $942.2\pm177.6$ & $676.1\pm370.9 $& $609.2\pm281.3$ &$\hgreen{ {999.3\pm\phantom{0}1.8}}$ & $775.0\pm381.8$ \\
\midrule
D-Pendulum & obs. & $\phantom{0}923.3\pm\phantom{0}\phantom{0}61.5$ & $\phantom{0}715.1\pm\phantom{0}215.0$& $\phantom{0}525.4\pm257.9$  &$\hgreen{ {1071.8\pm\phantom{0}87.1}}$ & $\phantom{0}160.8\pm\phantom{0}13.9$ \\
& act. & $2110.7\pm\phantom{0}\phantom{0}74.6$& $1280.9\pm\phantom{0}286.4$ & $\phantom{0}962.4\pm178.7$  & $\hgreen{ {2161.5\pm\phantom{0}36.0}}$ & $\phantom{0}301.2\pm\phantom{0}64.6$ \\
& env. & $7494.9\pm1189.1$ & $3023.9\pm\phantom{0}753.5$ & $2377.2\pm831.9$ & $\hgreen{ {8183.7\pm144.5}}$ & $\phantom{0}312.8\pm\phantom{0}50.5$ \\
& dom. & $7013.8 \pm\phantom{0} 850.6$ & $6103.9\pm1530.1$ & $2215.8\pm 915.6$  &$\hgreen{ {8174.2\pm178.2}}$&$1178.9\pm688.1$ \\
\bottomrule
\end{tabular}

\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

==> ICML19' (1)/ch4/table4c.tex <==
% !TEX root = ../draft.tex


%\begin{sidewaystable*}[h]
%\tiny
%%\begin{table*}[h]
%\centering
%\caption{Performance of 4 different implemented network architectures in terms of AUC score. All architectures are evaluated with 5 env.ironments and 3 noise type in each env.ironment. All performance are averaged over 12 random seeds.}
%\label{table: network}
%\vskip 0.15in
%\begin{center}
%\begin{small}
%\begin{sc}
%\begin{tabular}{l l c c c c c c c}
%\toprule
%\multicolumn{2}{l}{env. Name} & PPO & PPO-16 & SCN & SCN-16 & Ent-Reg & TRPO & TRPO-16 \\
%\midrule
%Walker2d & obs. & $\phantom{0}913.60 \pm 284.85$ &$1243.78 \pm 370.56$ & $1035.60 \pm 223.6$ & $1700.55 \pm 401.32$  & $\mathbf{2442.58 \pm 723.38}$& $859.36 \pm 229.26$ & $1082.75 \pm 223.01$\\
%& act. & $\phantom{0}845.53 \pm 251.44$ & $1181.57\pm 418.20$ & $\phantom{0}944.80\pm 229.14$ & $ 1167.21 \pm 464.64$ & $\mathbf{2843.93 \pm 1075.60}$ & $1259.50 \pm 310.19$& $1120.96 \pm 233.59$\\
%& env. & $2141.13\pm 558.51$ & $2337.43 \pm 633.70$ & $2180.54 \pm 458.85$ & $3050.92 \pm 805.76$ & $ \mathbf{3383.32 \pm 725.82}$&$2653.57 \pm 402.29 $& $ 2260.15 \pm 413.61$\\
%\midrule
%Hopper & obs. & $\phantom{0}592.64 \pm244.37$ & $\phantom{0}936.55\pm302.35$ & $\phantom{0}576.14\pm175.92$ & $\mathbf{\phantom{0}943.07\pm244.69}$ & $764.58 \pm 96.64$ &$ 643.81 \pm 107.21$&$ 758.73 \pm 230.97$\\
%& act. & $\phantom{0}608.97\pm167.64$ & $\phantom{0}994.14\pm296.43$ & $\phantom{0}550.59\pm124.00$ & $\mathbf{1060.89\pm299.25}$  &$890.78 \pm 108.65$&$ 683.03 \pm 121.76$&$ 810.15 \pm 270.39$\\
%& env. & $1241.58\pm438.72$ & $1971.61\pm545.31$ & $1277.84 \pm 314.80$ & $\mathbf{2109.00 \pm 651.54}$  &$1856.81\pm240.96$&$ 1638.70\pm383.67$&$1516.26\pm359.7 $\\
%\midrule
%Cheetah & obs. & $1030.37 \pm133.89$ & $1325.41 \pm 357.36$ & $\phantom{0}956.40\pm\phantom{0}59.20$ & $1116.58\pm287.87$ &$\mathbf{1382.32\pm 579.65}$&$ 1045.87 \pm 444.56$&$1072.59 \pm 370.11$ \\
%& act. & $\phantom{0}773.11\pm 177.45$ & $1099.38\pm399.32$ & $\phantom{0}771.21\pm160.61$ & $\phantom{0}986.17\pm412.87$ &$\mathbf{1316.98 \pm 782.09}$&$906.06\pm530.30$&$ 724.23\pm335.17$\\
%& env. & $986.17\pm412.87$ & $\mathbf{1406.86\pm152.14}$ & $\phantom{0}837.14\pm237.63$ & $1014.25\pm209.52$  \\
%\midrule
%Pendulum & obs. & $\phantom{0}139.51\pm\phantom{0}32.46$ & $\phantom{0}146.37\pm\phantom{0}39.84$ &$ \phantom{0}148.10\pm\phantom{0}74.93$ & $\mathbf{\phantom{0}177.42\pm\phantom{0}46.19}$ &$121.60\pm22.92$&$ 182.77\pm139.91$&$196.04\pm181.90$ \\
%& act. & $\phantom{0}362.68\pm\phantom{0}43.68$ & $\mathbf{\phantom{0}389.43\pm\phantom{0}18.98}$ & $\phantom{0}287.43\pm	122.27$ & $\phantom{0}302.52\pm\phantom{0}80.06$ &$363.60\pm26.77$&$201.04\pm112.84$&$145.10\pm119.71$ \\
%& env. & $\phantom{0}995.38\pm\phantom{00}8.00$ & $\mathbf{\phantom{0}998.74\pm\phantom{00}4.16}$ & $\phantom{0}820.64\pm344.93$ & $\phantom{0}975.81\pm\phantom{0}24.71$ &$994.43\pm5.23 $&$ 678.93\pm371.25$&$570.46\pm305.71$ \\
%\midrule
%D-Pendulum & obs. & $\phantom{0}923.25\pm\phantom{0}61.51$ &$ 1014.11\pm\phantom{0}78.40$ & $1051.29\pm150.97$ & $\mathbf{1093.81\pm121.60}$  &$ 956.06\pm66.94$&$ 715.10\pm214.98$&$ 632.78\pm287.37$\\
%& act. & $2110.66\pm\phantom{0}74.60$ & $\mathbf{2160.21\pm\phantom{0}44.23}$ & $2116.87\pm\phantom{0}70.79$ & $1944.06\pm\phantom{0}55.88$  &$ 2168.48\pm66.32$&$ 1280.97\pm286.35$&$869.91\pm298.98$\\
%& env. & $7494.92\pm 1189.12$ & $\mathbf{8036.72\pm 194.50}$ &$ 7997.09\pm 283.85$ & $7856.78\pm 601.89$ \\
%\bottomrule
%\end{tabular}
%\end{sc}
%\end{small}
%\end{center}
%\vskip -0.1in
%\end{sidewaystable*}


\begin{sidewaystable*}[t!]
\tiny
% %\begin{table*}[h]
\centering
\caption{Generalisation performance of different algorithms and architectures in terms of AUC score. All settings are evaluated with 5 environments and 4 noise types in each environment. All performance are averaged over 12 random seeds. The training settings that give top-$2$ performance within a test setting are highlighted in boldface. Welch's t-test ($p<0.05$) is used for significant testing. }
\label{table: network3}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\hspace{-0.5in}
\begin{tabular}{l l c c c c c c}
\toprule

\multicolumn{2}{l}{env. Name} & PPO & PPO-16 & PPO-SCN & PPO-SCN-16  & PPO-Ent & PPO-APRL \\
\midrule
Walker2d & obs. & $\phantom{0}966.2\pm 308.2$ & $ 1243.8 \pm 370.6$ & $1035.6\pm223.9$ & $\mathbf{1700.5\pm401.3}$&  $\mathbf{ 2442.6\pm \phantom{0}723.6 } $ & $\phantom{0}992.6\pm243.9$ \\
& act. & $\phantom{0}845.5\pm251.4$ & $ 1181.6\pm 418.2$ &$ \phantom{0}944.8\pm299.1$ & $\mathbf{1677.2\pm464.6}$ & $\mathbf{2843.9\pm 1075.6}$ & $\phantom{0}862.4\pm185.7$\\
& env. & $2141.1 \pm 558.5$& $ 2337.4 \pm 633.7$ &  $2180.5\pm458.9$ & $\mathbf{3050.9\pm805.8}$ & $\mathbf{3383.3 \pm \phantom{0} 725.8}$ & $2038.3\pm489.0$\\
& dom. & $2114.3 \pm 567.2$ & $ 2315.8\pm 618.4$ & $2166.6\pm447.6$ & $\mathbf{3039.5\pm810.8}$ & $\mathbf{3271.8 \pm \phantom{0} 740.4}$ & $1086.3\pm323.3$\\
\midrule
Hopper & obs. & $\phantom{0}592.6\pm 244.4$ & $\mathbf{\phantom{0}936.5\pm302.4}$ &  $\phantom{0}576.1\pm175.9$ &$\mathbf{\phantom{0}943.1\pm244.7}$ & $ \phantom{0}764.6\pm \phantom{0}96.6$ & $\phantom{0}624.0\pm175.0$ \\
& act. & $\phantom{0}609.0\pm167.6$ & $\mathbf{\phantom{0}994.1\pm 296.4}$ & $\phantom{0}550.6\pm124.0$ & $\mathbf{1060.9\pm299.3}$ & $ \phantom{0}890.8 \pm 108.7$ & $\phantom{0}724.7\pm181.7$ \\
& env. & $1241.6\pm438.7$ & $\mathbf{1971.6\pm545.3}$ & $1277.8\pm314.8$ & $\mathbf{2109.0\pm651.4}$ & $ 1856.8\pm 240.1$ & $1344.1\pm320.2$\\
& dom. & $ 1640.0\pm507.4$ & $\mathbf{1970.2 \pm 543.4}$ & $1277.1\pm317.2$ & $\mathbf{2111.3\pm650.8}$ & $ 1779.9\pm259.1$ & $1186.1\pm298.7$\\
\midrule
HalfCheetah & obs. & $1030.4\pm133.9$ & $ \mathbf{1325.4\pm\phantom{0}357.4}$ & $\phantom{0}956.4\pm\phantom{0}\phantom{0}59.2$ &$ 1116.6\pm\phantom{0}287.9$& $ \mathbf{1382.3\pm\phantom{0}579.7}$  & $\phantom{0}942.2\pm\phantom{0}87.0$ \\
& act. & $\phantom{0}773.1\pm 177.5$& $ \mathbf{1099.4\pm\phantom{0}399.3}$ & $\phantom{0}771.2\pm\phantom{0}160.6$ & $\mathbf{\phantom{0}986.2\pm\phantom{0}412.9}$ & $\mathbf{1316.9\pm\phantom{0}782.1}$  & $\phantom{0}685.5\pm166.6$\\
& env. & $1989.0\pm658.2$ & $\mathbf{3213.8 \pm 1417.0}$ & $\mathbf{2837.1 \pm \phantom{0}937.6}$ & $\mathbf{3014.3\pm 1109.5}$ & $\mathbf{2835.7\pm 1570.0}$ & $2202.6 \pm 927.7$\\
& dom. & $1871.0\pm583.5$ & $\mathbf{3035.4\pm 1309.8}$ & $ 2478.3\pm1129.5$ & $\mathbf{2730.3\pm1405.9}$ & $\mathbf{2677.5\pm 1454.6}$ & $2035.4\pm756.4$\\
\midrule
Pendulum & obs. & $129.5\pm\phantom{0}32.5$ & $\mathbf{146.4\pm 39.8}$ & $\mathbf{148.1\pm\phantom{0}74.9}$ & $\mathbf{177.4\pm46.2}$ &  $121.6\pm 22.9$ & $\phantom{0}57.4\pm\phantom{0}58.4$\\
& act. & $\mathbf{362.7\pm\phantom{0}43.7}$& $\mathbf{389.4\pm18.9}$ & $287.4\pm122.3$ & $302.5\pm80.1$ & $\mathbf{363.6\pm26.8}$ &  $156.8 \pm 165.1$ \\
& env. & $995.4\pm\phantom{00}8.0$ & $\mathbf{998.7\pm\phantom{0}4.2}$ &  $820.6\pm344.9$ & $975.8\pm24.7$ & $\mathbf{999.2\pm\phantom{0}3.6}$ & $381.8 \pm 401.4$\\
& dom. & $ 942.2\pm177.6$ &$\mathbf{998.7\pm\phantom{0}4.0}$ & $820.5\pm345.0$& $975.4\pm25.2$ & $\mathbf{999.9\pm\phantom{0}0.3}$ & $406.3\pm430.1$\\
\midrule
D-Pendulum & obs.& $\phantom{0}923.3\pm \phantom{00}61.5$ & $1014.1\pm\phantom{0}78.4$ & $\mathbf{1051.3\pm151.0}$ & $\mathbf{1093.8\pm121.6}$ & $ \phantom{0}956.1\pm\phantom{0}66.9$ & $\phantom{0}754.1\pm\phantom{0}\phantom{0}82.6$ \\
& act. & $2110.7\pm\phantom{00}74.6$ & $\mathbf{2160.2\pm\phantom{0}44.2}$  & $2016.9\pm\phantom{0}70.8$ & $1944.1\pm\phantom{0}55.9$ & $\mathbf{2168.5\pm\phantom{0}66.3}$ & $1917.0\pm\phantom{0}\phantom{0}64.6$ \\
& env. & $ 7494.9\pm1189.1$ & $\mathbf{8036.7\pm194.5}$ & $ \mathbf{7997.1\pm283.9}$ & $7856.8\pm601.9$ &  $5622.9\pm929.1$ & $3147.3\pm1157.1$ \\
& dom. & $7013.8\pm\phantom{0}850.6$ & $ \mathbf{8032.1\pm188.8}$ & $\mathbf{8006.9\pm278.6}$ & $7844.4\pm654.8$ & $  7436.7\pm696.6$ & $6667.0\pm1233.4$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{sidewaystable*}

==> ICML19' (1)/ch5/chap5.tex <==
% !TEX root = ../draft.tex

\section{Conclusion}
We contributed an analysis and set of benchmarks to investigate generalisation in deep RL.  The analysis showed that standard algorithms and architectures generalize poorly in the face of noise and environmental shift.  In particular, training and testing performance are often anti-correlated, so the standard practice of developing models with the aim of maximising training performance may be leading the community to produce less robust models. The results show that different off-the-shelf algorithms better address different aspects of generalisation performance, and various enhanced training strategies can also improve aspects of generalisation. However there is currently no generally good solution to all facets of generalisation, and new algorithms are needed.

%\doublecheck{It also highlights that development of an algorithm with good robustness to all noise types is an open question.}

==> ch5/chap5.tex <==
% !TEX root = ../draft.tex

\section{Conclusion}
We contributed an analysis and set of benchmarks to investigate generalisation in deep RL.  The analysis showed that standard algorithms and architectures generalize poorly in the face of noise and environmental shift.  In particular, training and testing performance are often anti-correlated, so the standard practice of developing models with the aim of maximising training performance may be leading the community to produce less robust models. The results show that different off-the-shelf algorithms better address different aspects of generalisation performance, and various enhanced training strategies can also improve aspects of generalisation. However there is currently no generally good solution to all facets of generalisation, and new algorithms are needed.

%\doublecheck{It also highlights that development of an algorithm with good robustness to all noise types is an open question.}
